Strategic Remote Attestation: Testbed for Internet-of-Things Devices and Stackelberg Security Game for Optimal Strategies

Internet of Things (IoT) devices and applications can have significant vulnerabilities, which may be exploited by adversaries to cause considerable harm. An important approach for mitigating this threat is remote attestation, which enables the defender to remotely verify the integrity of devices and their software. There are a number of approaches for remote attestation, and each has its unique advantages and disadvantages in terms of detection accuracy and computational cost. Further, an attestation method may be applied in multiple ways, such as various levels of software coverage. Therefore, to minimize both security risks and computational overhead, defenders need to decide strategically which attestation methods to apply and how to apply them, depending on the characteristic of the devices and the potential losses. To answer these questions, we first develop a testbed for remote attestation of IoT devices, which enables us to measure the detection accuracy and performance overhead of various attestation methods. Our testbed integrates two example IoT applications, memory-checksum based attestation, and a variety of software vulnerabilities that allow adversaries to inject arbitrary code into running applications. Second, we model the problem of finding an optimal strategy for applying remote attestation as a Stackelberg security game between a defender and an adversary. We characterize the defender's optimal attestation strategy in a variety of special cases. Finally, building on experimental results from our testbed, we evaluate our model and show that optimal strategic attestation can lead to significantly lower losses than naive baseline strategies.

==> history/testbed.tex <==
\section{Testbed Design and Development}\label{sec:design}

In our testbed, multiple IoT applications (or services) are running on multiple IoT devices. We implement and enable various software vulnerabilities (e.g., heap-based buffer overflow) in these applications so that adversaries can remotely compromise the devices by exploiting these vulnerabilities. As a result, adversaries can modify the {code} or the {control flow} of processes without crashing or restating them. 
% We also integrate multiple attestation methods (e.g., memory checksum, control-flow integrity) in the applications. Therefore, a verifier can remotely and dynamically verify the integrity of the vulnerable processes.
We also integrate memory checksum-based attestation method in the applications. Therefore, a verifier can remotely and dynamically verify the integrity of the vulnerable processes.

% \begin{itemize}
%     \item Vulnerable IoT projects running on different IoT devices
%     \item Adversaries can remotely compromise a device by exploiting software vulnerabilities
%     \item Adversaries can modify the \emph{code} or the \emph{control flow} of the running program without crashing
%     \item A verifier can remotely and dynamically verify the integrity of the running program using different attestation methods, e.g., memory checksum, control-flow integrity, etc.
% \end{itemize}

\subsection{Testbed Components}
A typical IoT testbed consists of several IoT devices running different IoT applications. In our testbed, we include two other nodes to perform the attacks (e.g., code injection, control flow alteration) on the applications and later to detect the attacks by verifying if devices are compromised. A simple testbed scenario is shown by Figure~\ref{fig:testbed_archi}.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=.8\textwidth]{figures/archi_remote_attest.pdf}
    \caption{Remote attestation testbed architecture.}
    \label{fig:testbed_archi}
\end{figure}

% \subsubsection{\textbf{System Components:}}
\paragraph{IoT Application Server Nodes}
We set up different IoT applications on individual nodes and implement vulnerabilities (e.g., a function vulnerable to format-string exploits) within the applications. Then, we debug all of these applications to find exploitation opportunities that can be utilized to perform code-injection attacks. Finally, we incorporate a memory-checksum generator, which can calculate a checksum whenever the process receives a challenge from an external verifier node.

\paragraph{Attacker Node}
The attacker node is a typical client node that can interact with the IoT application servers and execute various exploits (e.g., stack/heap-based buffer overflow). The purpose of the attacker node is to inject or alter software code within vulnerable applications without crashing the processes. In our testbed, the attacker node can launch attacks against all application server nodes. To tailor the attacks to the applications, the payload of each exploit is constructed based on debugging information that we previously obtained for each application.

\paragraph{Verifier Node}
The verifier node is responsible for performing remote attestation of the potentially compromised application server nodes using memory-checksum based attestation. % verification of the program memory or the program control-flow. 
For checksum based attestation, the verifier sends a challenge along with a random seed to the potentially compromised node and receives a response in return from the challenged device. Then, it sends the same challenge and same random seed to an identical, uncompromised device (in practice, this may be an isolated, trustworthy device) and receives its response.
Finally, it compares the two responses: if they match, the checksum is considered valid, and the device passed the attestation; otherwise, an attack is detected. 
% For, CFI, the verifier uses a monitoring program to monitor if the code execution flows normally and if that deviates from the control-flow graph (CFG).

% \subsubsection{\textbf{System Workflow:}}

% \subsubsection{\textbf{Attestation Algorithms:}}


\subsection{Testbed Development}
To experiment with various remote attestation strategies, we implement the following features in the testbed: start or terminate various IoT applications, exploit these applications from an attacker node, and generate challenge-response for remote attestation. 

\paragraph{Testbed Setup}
Our testbed use five Raspberry Pi 3 Model B+ device (two IoT application servers, an attacker, and two nodes for the verifier).
All devices run Raspbian Linux.
We incorporate two example IoT applications: %The IoT app servers are: 
an irrigation server\footnote{\url{https://github.com/NamedP1ayer/IrrigationServer}} and a smart home\footnote{\url{https://github.com/renair/smarthome}}.
% , and DNS Server\footnote{\url{https://github.com/Doredel/DNS_server_raspberrypi}}.

\paragraph{Enabling Vulnerabilities}
We disable certain security features of the Linux {kernel} and the {compiler} to enable {stack}- and {heap}-overflow based exploitation. By default, address space layout randomization (ASLR) is enabled on a Raspberry Pi. Therefore, we disable it to prevent a change of stack addresses each time we run a program. We also disable  {stack protection} and enable {code execution} for all memory pages while compiling and running the programs to facilitate exploitation simulation.

\paragraph{Exploitation Simulation}
%Exploitation requires software vulnerabilities within a program. Therefore, 
We debug all of the applications on the application server nodes to find stack- and heap-based vulnerabilities. Then, we create corresponding payloads on the attacker node. The attacker node sends a string to the server, which triggers the vulnerability and contains a shellcode to be injected into the process. We develop exploits that inject the shellcode into the code segment of the running processes. %a shellcode that can modify the instructions and workflow of the applications. 

% For example, in the general TCP Bind/Reverse shell execution, the string's whole buffer includes a NOP sled, shellcode, and the return address pointed to any address of the NOP sled. Our testbed consists of a stack and heap-based buffer overflow and ret-2-libc exploitation using TCP bind and reverse shells.

\paragraph{Integrity Verification Simulation}
There are several software-based remote attestation strategies to check the integrity of code, data, and control flow. In our testbed, we implement memory-checksum (sequential- and random-order checksum) as remote attestation strategies.

Checksum-based attestation requires an external trusted verifier. The verifier stores the same executable binary as the application server on another IoT device, which is assumed to be secure (e.g., isolated). 
The verifier can attest a potentially compromised device by sending the same challenge to both this device and the secure one and compare their responses.
%This secure devices is used to calculate the correct checksum for any challenge, which the potentially compromised 
%First, the verifier sends a challenge to the potentially-compromised IoT device, and in response, the device sends a computed checksum. Then, the verifier checks if this checksum matches the checksum that the secure device returns for the same challenge. 
%If the checksums do not match, an attack is detected. %the verifier ensures if the returned checksum matches the generated checksum received from the other identical application (using the same seed).


% \paragraph{\textbf{Testbed Interfacing:}}

==> tables/computation_overhead.tex <==
\begin{table}[!ht]
\caption{Computational Overhead Comparison}
\label{tab:computational_overhead}
\centering
\begin{tabular}{|c|c|}
\hline
\textbf{Attestation Strategy} & \textbf{\begin{tabular}[c]{@{}c@{}}Required Time (approx.)\\ (in seconds)\end{tabular}} \\ \hline\hline
Checksum & 0.12509 \\ \hline
CFI (level 0) & 0.13352 \\ \hline
CFI (level 1) & 42.45723 \\ \hline
\end{tabular}
\end{table}

==> tables/payoff_table.tex <==
\begin{table}[ht]
\centering
\caption{Example: Attacker-Defender Payoffs}
\label{tab:payoffs}
\begin{tabular}{|c|c||c|c|}
\hhline{|-|-||-|-|}
\textbf{Players}          &                  & \multicolumn{2}{c|}{\textbf{Attacker}} \\ \hhline{|-|-||-|-|}
                          & \textbf{Actions} & Attack      & Not Attack      \\ \hhline{==::==}
\multirow{2}{*}{\textbf{Defender}} & Attestation         & 2,-2        & -1,1            \\ \hhline{|~|-||-|-|} 
                          & No-Attestation      & 0,5         & 5,0             \\ \hhline{|-|-||-|-|}
\end{tabular}
\end{table}
